Towards Large-Pose Face Frontalization in the Wild

Despite recent advances in face recognition using deep learning, severe accuracy drops are observed for large pose variations in unconstrained environments. Learning pose-invariant features is one solution, but needs expensively labeled large-scale data and carefully designed feature learning algorithms. In this work, we focus on frontalizing faces in the wild under various head poses, including extreme profile views. We propose a novel deep 3D Morphable Model (3DMM) conditioned Face Frontalization Generative Adversarial Network (GAN), termed as FF-GAN, to generate neutral head pose face images. Our framework differs from both traditional GANs and 3DMM based modeling. Incorporating 3DMM into the GAN structure provides shape and appearance priors for fast convergence with less training data, while also supporting end-to-end training. The 3DMM-conditioned GAN employs not only the discriminator and generator loss but also a new masked symmetry loss to retain visual quality under occlusions, besides an identity loss to recover high frequency information. Experiments on face recognition, landmark localization and 3D reconstruction consistently show the advantage of our frontalization method on faces in the wild datasets.

==> frontalization_intro.tex <==
\section{Introduction}
Frontalization of face images observed from extreme viewpoints is a problem of fundamental interest in both human and machine facial processing and recognition. Indeed, while humans are innately skilled at face recognition, newborns do not perform better than chance on recognition from profile views \cite{Turati_etal_2008}, although this ability seems to develop rapidly within a few months of birth \cite{Fagan_1976}. Similarly, dealing with profile views of faces remains an enduring challenge for computer vision too. The advent of deep convolutional neural networks (CNNs) has led to large strides in face recognition, with verification accuracy surpassing human levels \cite{SunCVPR14,Sunnips2014} on datasets such as LFW. But even representations learned with state-of-the-art CNNs suffer for profile views, with severe accuracy drops reported in recent studies \cite{Kanmeina16,CFP}. Besides aiding recognition, frontalization of faces is also a problem of independent interest, with potential applications such as face editing, accessorizing and creation of models for use in virtual and augmented reality.

\begin{figure}[t!]
\begin{center}
\includegraphics[width=0.47\textwidth]{teasor_wild.pdf}
\end{center}
\vspace{-3mm}
\caption{The proposed FF-GAN framework. Given a non-frontal face image as input, the generator produces a high-quality frontal face. Learned 3DMM coefficients provide global pose and low frequency information, while the input image injects high frequency local information. A discriminator distinguishes generated faces against real ones, where high-quality frontal faces are considered real. A face recognition engine is used to preserve identity information. The output is a high quality frontal face that retains identity.}
\vspace{-3mm}
\label{fig:concept}
\end{figure}

In recent years, CNNs have leveraged the availability of large-scale face datasets to also learn pose-invariant representations for recognition, using either a joint single framework \cite{MasiCVPR16} or multi-view pose-specific networks \cite{ZhuNIPS2014,Kanmeina16}. Early works on face frontalization in computer vision rely on frameworks inspired by computer graphics. The well-known 3D Morphable Model (3DMM) \cite{3dmm} explicitly models facial shape and appearance to match an input image as closely as possible. Subsequently, the recovered shape and appearance can be used to generate a face image under novel viewpoints. Many 3D face reconstruction methods \cite{roth2015,zhu2016face,rothpami} build upon this direction by improving speed or accuracy. Deep learning has made inroads into data-driven estimation of 3DMM models too \cite{ZhuNIPS2014,Kanmeina16,jourabloo2017pose}, circumventing some drawbacks of early methods such as over-reliance on the accuracy of 2D landmark localization \cite{xiang_pami_cdm_2015,xiang_cor_2014}. Due to restricted Gaussian assumptions and nature of losses used, insufficient representation ability for facial appearance prevents such deep models from producing outputs of high quality. While inpainting methods such as \cite{ZhuXYCVPR15} attempt to minimize the impact on quality due to self-occlusions, they still do not retain identity information.

In this paper, we propose a novel generative adversarial network framework FF-GAN that incorporates elements from both deep 3DMM and face recognition CNNs to achieve high-quality and identity-preserving frontalization, using a single input image that can be a profile view up to $90^{\circ}$. Our framework targets more on face-in-the-wild conditions which show more challenge on illumination, head pose variation, self-occlusion and so on. To the best of our knowledge, this is the first face frontalization work that handles pose variations at such extreme poses.

Noting the challenge of purely data-driven face frontalization, Section \ref{sec:reconstruction} proposes to enhance the input to the GAN with 3DMM coefficients estimated by a deep network. This provides a useful prior to regularize the frontalization, however, it is well-known that deep 3DMM reconstructions are limited in their ability to retain high-frequency information. Thus, Section \ref{sec:generation} proposes a method to combine 3DMM coefficients with the input image to generate an image that maintains both global pose accuracy and retains local information present in the input image. In particular, the generator in our GAN produces a frontal image based on a reconstruction loss, a smoothness loss and a novel symmetry-enforcing loss. The aim of the generator is to fool the discriminator, presented in Section \ref{sec:discrimination}, into being unable to distinguish the generated frontal image from a real one. However, neither the 3DMM that loses high-frequency information, nor the GAN that only aligns domain-level distributions, suffice to preserve identity information in the generated image. To retain identity information, Section \ref{sec:recognition} proposes to use a recognition engine to align the feature representations of the generated image with the input. A balanced training with all the above objectives results in high-quality frontalized faces that preserve identity.

We extensively evaluate our framework on several well-known datasets including Multi-PIE, AFLW, LFW, IJB-A and CFP. In particular, Section \ref{sec:experiments} demonstrates that the face verification accuracy on LFW dataset that uses information from our frontalized outputs exceeds previous state of the art. We observe even larger improvements on the Multi-PIE dataset especially for the viewpoints beyond $45^\circ$ and being the sole method among recent works to produce high recognition accuracies for $75^\circ$-$90^\circ$. We present ablation studies to analyze the effect of each module and several qualitative results to visualize the quality of our frontalization.

To summarize, our key contributions are:
\vspace{-0.2cm}
\begin{tight_itemize}
\item A novel GAN-based end-to-end deep framework to achieve face frontalization even for extreme viewpoints.
\item A deep 3DMM model to provide shape and appearance regularization beyond the training data.
\item Effective symmetry-based loss and smoothness regularization that lead to generation of high-quality images.
\item Use of a deep face recognition CNN to enforce that generated faces satisfy identity-preservation, besides realism and frontalization.
\item Consistent improvements on several datasets across multiple tasks, such as face recognition, landmark localization and 3D reconstruction.
\end{tight_itemize}




